DyLink2Vec: Effective Feature Representation for Link Prediction in Dynamic Networks

The temporal dynamics of a complex system such as a social network or a communication network can be studied by understanding the patterns of link appearance and disappearance over time. A critical task along this understanding is to predict the link state of the network at a future time given a collection of link states at earlier time points. In existing literature, this task is known as link prediction in dynamic networks. Solving this task is more difficult than its counterpart in static networks because an effective feature representation of node-pair instances for the case of dynamic network is hard to obtain. To overcome this problem, we propose a novel method for metric embedding of node-pair instances of a dynamic network. The proposed method models the metric embedding task as an optimal coding problem where the objective is to minimize the reconstruction error, and it solves this optimization task using a gradient descent method. We validate the effectiveness of the learned feature representation by utilizing it for link prediction in various real-life dynamic networks. Specifically, we show that our proposed link prediction model, which uses the extracted feature representation for the training instances, outperforms several existing methods that use well-known link prediction features.

==> ml_author_question_answer.tex <==
\section{MLJ Contribution Information Sheet}
{\em 1. What is the main claim of the paper? Why is this an important contribution to the machine learning literature?}

\noindent \textbf{Our Answer:}  The temporal dynamics of a complex system such as a social network or a
communication network can be studied by understanding the patterns of link
appearance and disappearance over time. A critical task along this
understanding is to predict the link state of the network at a future time
given a collection of link states at earlier time points. In existing literature,
this task is known as link prediction in dynamic networks. In this work, we propose \alg, a scalable method for finding the metric embedding of arbitrary node-pairs (both edges or non-edges) of a  
dynamic network with many temporal snapshots. This work is different from existing 
works of representation learning on graphs in two ways:
first, existing works find the embedding of vertices whereas we consider embedding
of arbitrary node-pairs; second, our work considers a dynamic network, which has
many temporal snapshots, whereas existing works consider only a static network. Therefore, 
our embedding method is particularly suitable for link forecasting
in a dynamic networks, and thus, would be an important contribution to the machine learning literature.\\

\noindent {\em 2. What is the evidence you provide to support your claim? Be precise.}

\noindent  \textbf{Our Answer:} We present following evidences: 
\begin{itemize}
\item We validate the effectiveness of our representation learning method (\alg) by utilizing it for link prediction on four real-life dynamic networks- {\em Enron}, {\em Collaboration}, and two version of {\em Facebook} networks.
\item We compare the quality of embedding generated from \alg\ (our algorithm) with multiple state-of-the-art methods for dynamic link prediction task. Our comparison results show that the proposed method is superior than all the competing methods.
\end{itemize}

\noindent {\em 3. What papers by other authors make the most closely related contributions, and how is your paper related to them?}

\noindent  \textbf{Our Answer:} A key challenge of link prediction in a dynamic network is to find a suitable feature representation of the node-pair instances which are used for training the prediction model. For the static link prediction problem, various topological metrics (common neighbors, Adamic-Adar, Jaccard's coefficient) are used as features, but they can not be extended easily for the dynamic setting having multiple snapshots of the network. In this work, we propose a very general method for constructing unsupervised feature representation in 
dynamic setting. The following papers also provide methods for generating useful node-pair (edge) feature representation, and thus they are related to our work. 
\begin{itemize}
\item Temporal Link prediction using matrix and tensor factorization by D.M. Dunlavy, T. G. Kolda, and E. Acar, in ACM Trans. Knowl. Discov. Data, 2011

\item Link prediction using time series of neighborhood-based node similarity scores by
G{\"u}ne{\c{s}}, {\.I}smail and G{\"u}nd{\"u}z-{\"O}{\u{g}}{\"u}d{\"u}c{\"u}, {\c{S}}ule and {\c{C}}ataltepe, Zehra, in
Data Mining and Knowledge Discovery, 2015

\item DeepWalk: Online Learning of Social Representations by
Perozzi, Bryan and Al-Rfou, Rami and Skiena, Steven, in Proc.
of SIGKDD, 2014. 

\end{itemize}

\noindent {\em 4. Have you published parts of your paper before, for instance in a conference? If so, give details of your previous paper(s) and a precise statement detailing how your paper provides a significant contribution beyond the previous paper(s).}

\noindent \textbf{Our Answer:} No, we did not publish parts of our paper anywhere.

